Medical Entity Disambiguation Using Graph Neural Networks

Medical knowledge bases (KBs), distilled from biomedical literature and regulatory actions, are expected to provide high-quality information to facilitate clinical decision making. Entity disambiguation (also referred to as entity linking) is considered as an essential task in unlocking the wealth of such medical KBs. However, existing medical entity disambiguation methods are not adequate due to word discrepancies between the entities in the KB and the text snippets in the source documents. Recently, graph neural networks (GNNs) have proven to be very effective and provide state-of-the-art results for many real-world applications with graph-structured data. In this paper, we introduce ED-GNN based on three representative GNNs (GraphSAGE, R-GCN, and MAGNN) for medical entity disambiguation. We develop two optimization techniques to fine-tune and improve ED-GNN. First, we introduce a novel strategy to represent entities that are mentioned in text snippets as a query graph. Second, we design an effective negative sampling strategy that identifies hard negative samples to improve the model's disambiguation capability. Compared to the best performing state-of-the-art solutions, our ED-GNN offers an average improvement of 7.3% in terms of F1 score on five real-world datasets.

==> embedding.tex <==
\section{Heterogeneous Graph Neural\\ Network Design}
\label{sec:gnn}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.9\columnwidth]{figures/gnn.pdf} 
\caption{The overall architecture of \gnn.}
\label{fig:gnn}
\end{center}
\end{figure*}

In this section, we present our metapath-based graph neural network \gnn\ based on~\cite{HAN,MAGNN} for medical entity disambiguation. The basic idea is to represent a medical KG as a HIN $\mathcal{H}_R$ = ($\mathcal{V}_R$, $\mathcal{E}_R$), where nodes correspond to medical entities and edges correspond to relationships between those entities. Such a heterogeneous GNN potentially enriches the representations of the targeted node types (e.g., admission, finding, drug, etc.) for entity disambiguation. As shown in Figure~\ref{fig:gnn}, the overall framework of \gnn\ consists of three layers: term embedding, neighbor aggregation, and metapath aggregation. First, \gnn\ takes as input a graph $\mathcal{H}_R$. Second, we use word embedding-based methods to generate the initial term embeddings of the nodes in $\mathcal{H}_R$. Third, we aggregate the information of metapath-guided neighbors to learn the embeddings of each metapath instance. After that, we combine all metapath embeddings of the targeted nodes along with their respective features as the representation of each node. Figure~\ref{fig:gnn} illustrates the embedding generation of a single node.

\subsection{Term Embedding Layer}
\label{sec:gnn:term}

In principle, each node in a HIN can be associated with different types of attributes, capturing the semantic information of the graph. In the case of our medical KG, every node may be associated with a set of attributes, which describe this node (e.g., name, synonyms, definition). We assume that all nodes are associated with a name attribute, consisting of one or more words (e.g., ``exfoliative dermatitis'') which we call a \textit{composite term}. However, our \gnn\ can be easily extended to capture multiple types of node attributes, with different dimensions of feature vectors. Namely, a type-specific linear transformation can be used to project different types of node attributes into the same latent vector space.

\textbf{Word Embedding.} 
As described above, all attributes (i.e., terms) are constituted of domain-specific words. One can leverage state-of-the-art deep learning-based embedding methods such as BERT~\cite{bert} or ELMo~\cite{elmo} to produce  high-quality word embeddings. In this work, we choose a high-quality pre-trained medical language model on PubMed abstracts and clinical notes (MIMIC-III)~\cite{peng2019transfer}. Alternatively, one can choose a neural architecture to train a model in an unsupervised manner.

% We choose a character-level embedding method~\cite{bojanowski2016enriching} to train word embeddings for the vocabulary used in the medical KG. The reasons are the following: pre-trained embeddings may not be suitable for the medical domain, where the vocabulary contains tokens with highly specialized semantics (e.g., finding site). Moreover, character-level embeddings are more robust to out-of-vocabulary words, as they leverage possible substrings of the word to approximate its embedding. In this case, training a domain-specific embedding leads to improved performance in scenarios such as entity disambiguation where long-tail vocabularies are common and typographical errors are widespread.

\textbf{Term Embedding.} 
We then aggregate the word embeddings to generate the term embeddings. For this aggregation, we use the Smooth Inverse Frequency (SIF) sentence embedding model~\cite{DBLP:conf/iclr/AroraLM17}, which performs a weighted average of the constituent word embeddings. The weight $f(w)$ for the embedding of a word $w$ is $f(w)$ = $a/(a + p(w))$, where $a$ is a hyperparameter and $p(w)$ is the normalized unigram frequency of $w$ in the text corpus. This model was chosen since it is simple, but with comparable effectiveness to other more complex and much harder to train models for text similarity, sentence entailment and other NLP tasks. After applying this aggregation, the resulting term embedding is used as the initial state $h_v^{\text{attr}}$ of each node.


\subsection{Neighbor Aggregation Layer}
\label{sec:gnn:neighbors}

Given a metapath $P_r$, the neighbor aggregation layer learns the structural and semantic information embedded in the target node and the metapath-based neighbors by encoding the metapath instances of $P_r$. We continue to use the network schema in Figure~\ref{fig:schema} to illustrate this process. Here we describe how to obtain the embedding of the target node $F_1$ based on the instances of a metapath $P_r$ = DAF. Let $P_r(v,u)$ be a metapath instance of $P_r$ connecting the target node $v$ (i.e., $F_1$) and the source node $u$ (i.e., $D_1$). We first use the linear encoder, an extension to the mean encoder, to aggregate the node vectors along the metapath instance (i.e., $D_1$$A_1$$F_1$) into a single vector.

\begin{equation}
h_{P_r(v,u)} = W_p \cdot \text{MEAN}(\{h_i^{\text{attr}}, \forall i \in P_r(v,u)\}),
\label{eq.1}
\end{equation}

\noindent where $W_p$ is the parametric weight matrix.

After encoding the metapath instances into vector representations, we exploit a graph attention mechanism~\cite{DBLP:conf/iclr/VelickovicCCRLB18} to weighted sum the metapath instances of $P_r$ with respect to the target node $F_1$. The intuition is to learn the importance of different neighbors of $F_1$. Note that the importance of a pair of nodes is asymmetric. This way we can preserve the asymmetry property of the heterogeneous graph. We model this by learning a normalized importance weight $\alpha^{P_r}_{v,u}$ for each metapath instance.

\begin{equation}
\alpha^{P_r}_{v,u} = \frac{\exp\big(\sigma\big(\boldsymbol{a}^{\intercal}[h^{\text{attr}}_{v}\parallel h_{P_r(v,u)}]\big)\big)}{\sum_{s \in N^{P_r}_{v}}\exp\big(\sigma\big(\boldsymbol{a}^{\intercal}[h^{\text{attr}}_{v}\parallel h_{P_r(v,s)}]\big)\big)},
\label{eq.2}
\end{equation}

\noindent where $\sigma$ is an activation function, $\boldsymbol{a}$ is a parameterized attention vector for metapath $P_r$, and $\parallel$ denotes the concatenation. We obtain $\alpha^{P_r}_{v,u}$ for all metapath-based neighbors (i.e., $D_1$, $D_2$, and $D_3$) of $F_1$ (in Figure~\ref{fig:gnn}). Consequently, we use them to compute the representations of the metapath instances (i.e., $D_1$$A_1$$F_1$, $D_2$$A_2$$F_1$, and $D_2$$A_3$$F_1$) related to $F_1$.

\begin{equation}
h^{P_r}_{v} = \parallel^{K}_{k=1}\sigma\Big(\sum_{u \in N^P_v}[\alpha^{P_r}_{v,u}]h_{P_r(v,u)}\Big),
\label{eq.3}
\end{equation}

\noindent where $[\alpha^{P_r}_{v,u}]$ denotes the normalized importance of metapath instance to node $v$ at the $k$-th attention head. Here the attention mechanism is extended to multiple heads in order to stabilize the learning process and to reduce the high variance introduced by the heterogeneous graphs.

In summary, given a set of metapath $\mathcal{P}_R$ = \{$P_1$, $P_2$, $\cdots$, $P_r$\} in which the target node type $T\in$ $\mathcal{T}$ and all initial feature vectors $h_v^{attr}$, for every $v\in \mathcal{V}_R$, the neighbor aggregation of \gnn\ generates $|\mathcal{P}_R|$ metapath-based vector representations of the target nodes $v\in \mathcal{V_T}$, denoted as \{$h^{P_1}_{v}$, $h^{P_2}_{v}$, $\cdots$, $h^{P_r}_{v}$\}.


\subsection{Metapath Aggregation Layer}
\label{sec:gnn:metapath}

Generally, each node $v\in$ $\mathcal{V}_R$ contains rich semantic information and the embeddings from the neighbor aggregation can only reflect nodes from one aspect. To learn a more comprehensive node embedding, we now fuse different neighbor aggregations from different metapaths using the attention mechanism to assign different weights to different metapaths. Similar to Equation~\ref{eq.2}, we model this by learning an importance weight $\beta^{P_r}_v$ for each metapath $P_r$ to the target node $v$.

\begin{equation}
\beta^{P_r}_v = \frac{\exp\big(\sigma\big(\boldsymbol{\beta}^{\intercal}h^{P_r}_{v}\big)\big)}{\sum_{P_s \in \mathcal{P}_{R}}\exp\big(\sigma\big(\boldsymbol{\beta}^{\intercal}h^{P_s}_{v}\big)\big)},
\label{eq.4}
\end{equation}

\noindent where $\sigma$ is an activation function, and $\boldsymbol{\beta}$ is an attention vector for neighbor aggregates. It indicates the relative importance of metapath $P_r$ to the target node type $T$. In Figure~\ref{fig:gnn}, the target node $F_1$ has two vector representations $h^{P_1}_{v}$ and $h^{P_2}_{v}$ represent the neighbor aggregations based on DAF and DIF, respectively. Once $\beta^{P_r}_v$ is computed for each $P_r$ associated to the targeted node type, we weighted sum all the metapath-based node vectors of $v$ to produce the final vector representation $h_v$ of $v$.

\begin{equation}
h_v = \sum_{P_r \in P_{R}} \beta^{P_r}_v h^{P_r}_{v} 
\label{eq.5}
\end{equation}


\subsection{Training}
\label{sec:gnn:training}

After applying three layers introduced in the previous subsections, we obtain the final node representations, which can then be used for different downstream tasks, including entity disambiguation. In this work, we optimize the model weights by minimizing the following loss function through negative sampling:
\begin{equation}
\begin{aligned}
\mathcal{L} = & -\sum_{(u,v)\in \Omega} log (\sigma (\textbf{\textit{h}}^\top_u \textbf{\textit{h}}_v)) -   \sum_{(u,v)\in \Omega^-} log(\sigma (\textbf{\textit{h}}^\top_u \textbf{\textit{h}}_{v'})),
\end{aligned}
\label{eq:loss}
\end{equation}
where $\sigma$($\cdot$) is the sigmoid function, $\Omega$ is the set of observed (positive) node pairs, and $\Omega^-$ is the set of negative node pairs sampled from all unobserved node pairs. In our entity disambiguation scenario, a positive node pair consists of one node representing an entity in the text snippet and one node representing its corresponding matching node in the medical KG, respectively.
